Robust Closed-form Framework for Drag-Propulsive Control of Formation Flight

To conserve propellant, Distributed Space Systems (DSS) can leverage environmental forces to produce low cost relative forces, such as atmospheric drag in Low Earth Orbit (LEO). This work maximizes this strategy by developing robust, closed-form algorithms for optimal "hybrid" control, defined here as complementing the magnitude and directionality deficiencies of differential drag with the superior control authority of propulsive maneuvers within the same control window. The use of drag introduces a significant source of dynamic uncertainty to the control problem, primarily from inaccurate atmospheric density modelling. This paper develops a robust control architecture that periodically re-solves the remaining drag maneuver plan in a diminishing horizon policy, rejecting operational and navigation errors while retaining the cost savings offered by differential drag. The approach is built upon reachable set theory, a control analysis technique that provides conditions for optimality for Linear Time Variant (LTV) systems with norm-like cost functions and optimally decouples hybrid control into separate propulsive and differential drag sub-problems. The optimality conditions are leveraged to prove the asymptotic Lyapunov stability of ideal reachable set-based control solutions and derive error bounds on this stability. A covariance analysis on the primary sources of error in hybrid control determines that the dominating source of uncertainty is the atmospheric density model. This conclusion allows the bounds on Lyapunov stability to be completely met by simply conditioning the atmospheric density value used in the control solutions. The derived Lyapunov stability bounds and performance of the algorithm are demonstrated experimentally in high fidelity full-force orbital simulations of the upcoming Space Weather Reconfigurable Multiscale Experiment (SWARM-EX) mission.

==> backup.tex <==
\subsection{Reachable Set Theory}

The proposed robust architecture is built upon the provably-optimal closed-form solver of Eq. \ref{eq: hybrid control problem} from previous work by the authors, and the overall approach is summarized here in brevity. A more detailed derivation is given in Appendix \ref{}. Reachable set theory primarily considers two sets under the dynamics in Eq. \ref{eq: dynamics}: the set $S(c,T)$ of all $\Delta \delta \boldsymbol{\alpha}$ that can be reached by a single maneuver $u$ of arbitrary cost $c$ over times in the control window $T$ and the set $S^*(c,T)$ of all $\Delta \delta \boldsymbol{\alpha}$ that can be reached by $k \geq 1$ maneuvers $\boldsymbol{u}_i$ at times $t_i \in T$ of combined cost greater than $c$, given as
\begin{align}
    S(c,T) = \{\Delta \delta \boldsymbol{\alpha}:& \Delta \delta \boldsymbol{\alpha} = \boldsymbol{\Gamma}(t) \boldsymbol{u}, \left\|\boldsymbol{u}\right\|_{2} \leq c, t \in T \} \label{eq: RST S} \\
    S^*(c,T) = \{\Delta \delta \boldsymbol{\alpha}:& \Delta \delta \boldsymbol{\alpha} = \Sigma^{k}_{i=1} \boldsymbol{\Gamma}(t_i)\boldsymbol{u}_i, t_i \in T, \label{eq: RST S*} \\
    & \hspace{20mm} \left\|\boldsymbol{u}_i \right\|_{2} \leq c_i, \Sigma^{k}_{i=1} c_i = c \} \nonumber
\end{align}
It can be seen that $S^*$ is a linear combination, and therefore convex hull, of the $\Delta \delta \boldsymbol{\alpha}$ in $S$. Given that the norm-like cost function scales linearly with magnitude, the $c$ that scales $S^*$ until its boundary contains the reconfiguration $\Delta \delta \boldsymbol{\alpha}$ is the minimum or optimal cost $\delta v_{\text{min}}$.

Several observations about this formulation establish the structure of the hybrid solver \cite{chernick}. The 2$n$-dimensional (2$n$D) reconfiguration can be broken down into $n$ 2D planes, where the 2D plane that contains the highest $\delta v_{\text{min}}$, known as the dominant plane, is driven by a specific dimension, known as the dominance case. The different dominance cases are distinguished by distinct contours of the reachable set that intersect $\Delta \delta \boldsymbol{\alpha}$ at minimum cost. The minimum cost $\delta v_{\text{min}}$ for each dominance case is found as the solution to
\begin{equation} \label{eq: delta-v min}
    \hspace{-2mm}
    \text{maximize: } \frac{\boldsymbol{\eta}^{\text{T}} \Delta \delta \boldsymbol{\alpha}}{\max_{t \in T} \left( \max_{||\boldsymbol{u}|| \leq 1 } \left( \boldsymbol{\eta}^{\text{T}} \boldsymbol{\Phi}^{J_2}(t) \boldsymbol{B}(t) \boldsymbol{u} \right) \right) },
\end{equation}
\noindent where the cominance case contour is defined by the outward normal $\boldsymbol{\eta}$ of the supporting hyperplane \cite{koenig_impulse}. Furthermore, the dominance case optimal maneuver times $T_{\text{opt}}$, resulting from the denominator of Eq. \ref{eq: delta-v min}, occur visually at points on $S^*$, defined by $\boldsymbol{\eta}$, that share a boundary with $S$. Restricting maneuver solutions to these times enables the creation of closed-form solutions. However, given the coupled dynamics between 2D planes, the full 2$n$D reconfiguration $\delta v_{\text{min}}$ must be greater or equal to that of the dominance case and matches only when $\Delta \delta \boldsymbol{\alpha}$ is reachable at the dominance case $\delta v_{\text{min}}$, meaning $\Delta \delta \boldsymbol{\alpha}$ lies on the boundary of $S^*(\delta v_{\text{min}},T_{\text{opt}})$ in the dominant plane and within $S^*(\delta v_{\text{min}},T_{\text{opt}})$ in the non-dominant planes.

Applying this methodology to the hybrid control problem in Eq. \ref{eq: hybrid control problem}, the ROE can be conveniently arranged into 3 2D planes to match the decoupling found in $\boldsymbol{B}$: the $\Delta \delta \boldsymbol{a}$ plane ($\Delta \delta a$, $\Delta \delta \lambda$), the $\Delta \delta \boldsymbol{e}$ plane, and the $\Delta \delta \boldsymbol{i}$ plane. This arrangement enables the IP and OOP reconfiguration sub-problems to be analyzed and solved independently, while still accounting for the J2 coupling present in $\boldsymbol{\Phi}^{J_2}$. Propulsive and differential drag control can also be decoupled into independent sub-problems. Because drag is a zero-cost maneuver, the dominance cases and corresponding $\boldsymbol{\eta}$ that result from the propulsive analysis can also be applied to the differential drag reachable set to identify optimal drag profiles, or the modulation of differential attitude over time. Figure \ref{} illustrates this approach visually for the IP reconfiguration.



\noindent Chernick, Hunter, and D'Amico leveraged the simplicity of the propulsive ROE reachable sets to identify three IP dominance cases ($\delta a$, $\delta \lambda$, and $\delta e$), with tangential-only optimal maneuvers, and one OOP dominance case ($\delta i$), with normal-only optimal maneuvers, to produce analytical expressions of the corresponding $\delta v_{\text{min}}$ and $T_{\text{opt}}$. The IP $\delta v_{\text{min}}$, relevant for hybrid control, are given as
\begin{align} 
    \delta v_{\text{min}, \delta a} &= \pm \frac{1}{2}n_c a_c  \Delta \delta a  \label{eq: Chernick dv min da}\\
    \delta v_{\text{min}, \delta \lambda} &= \frac{\pm (m \Delta \delta\lambda - \Delta  \delta a) }{ \Delta \delta a_0} \label{eq: Chernick dv min dl}\\
    \delta v_{\text{min}, \delta e} &= \frac{1}{2} n_c ||a_c \Delta \delta \boldsymbol{e}||_2 
    \label{eq: Chernick dv min de}
\end{align}
\noindent where $\Delta \delta a_0$ defines the pseudostate achieved by a unitary tangential impulse at $t_0$, $\Delta \delta a$-$\Delta \delta \lambda$ slope $m = 2/(\Phi_{21}^{J_2}(t_f-t_0))$, and $\delta v_{\text{min}}$ denotes a propulsive delta-v minimum. The authors applied the $\boldsymbol{\eta}$ from the IP propulsive dominance cases to the ROE differential drag reachable sets to find the optimal drag, or differential attitude, profile associated with each single dominance case and the analytical effect of the profile on the dominance case's $\delta v_{\text{min}}$, given as
\begin{align} 
    \Delta \delta v_{\text{min},\delta a} \hspace{-0.5mm} &= \hspace{-0.5mm} \frac{1}{2}a_{c}^{2}n_{c}^{2} \Delta B^{\rho} \Delta t \label{eq: drag da} \\
    \Delta \delta v_{\text{min},\delta \lambda} \hspace{-0.5mm} &= \hspace{-0.5mm} a_{c}^{2}n_c \Delta B^{\rho}\frac{\Phi_{21}^{J_2}m(2 \tau \Delta t \hspace{-0.5mm} - \hspace{-0.5mm} 2t\Delta t \hspace{-0.5mm} - \hspace{-0.5mm} \Delta t^2) \hspace{-0.5mm} - \hspace{-0.5mm} 2\Delta t}{2a_c \Delta \delta a_0} \label{eq: drag dl}\\
    \Delta \delta v_{\text{min},\delta e} \hspace{-0.5mm} &= \hspace{-0.5mm} \frac{a_{c}^{2}n_{c}^{2}\Delta B^{\rho}}{\pi} \Delta t \label{eq: drag de}
\end{align}
\noindent where $\tau = t_f - t_0$, $\Delta \delta v_{\text{min}}$ denotes the change in the delta-v minimum due to using a drag profile, $t$ and $\Delta t$ are the start time and length of a single dominance case drag profile, and the periodic effects in $\Delta \delta v_{\text{min},\delta e}$ are approximated as linear. The $T_{\text{opt}}$ are used to create maneuver plans in closed-form. By limiting possible maneuver times to those in $T_{\text{opt}}$ for all dominance cases, the authors designed a solver that creates provably-optimal or near-optimal hybrid control solutions in in linear time and with comparable final state accuracy to impulsive-only control under ideal maneuvering. This solver will be used in this work to understand the impact of different sources of error on the performance of hybrid control.


\subsection{Closed-form Hybrid Solver}

The resulting hybrid solver developed by the authors solves the full reconfiguration in three closed-form sequential steps: differential drag, OOP propulsive, and IP propulsive. $\Delta \delta \boldsymbol{\alpha}$ is modified by the expected effect of each maneuver plan to minimize IP/OOP coupling. The differential drag solution must address the possibility that the full reconfiguration optimal drag profile results in multiple dominance cases with equal $\delta v_{\text{min}}$ due to the use of zero-cost maneuvers. Therefore, an optimal composite profile arranges the single dominance case profiles in the control window to have a negligible effect on the non-affiliated IP dominance cases and finds the optimal combination by comparing the effect of each on the IP $\delta v_{\text{min}}$. The basic structure of the composite drag profile is illustrated in Figure \ref{}.



The base propulsive solver takes advantage of the linear relationship between Eq. \ref{eq: RST S} and \ref{eq: RST S*}. The solver first identifies the dominance case of the IP/OOP sub-problem and finds $S(\delta v_{\text{min}},T_{\text{opt}})$, the set of pseudostate effects $\Delta \delta \boldsymbol{\alpha}_i$ for optimal propulsive maneuvers $i$ of magnitude $\delta v_{\text{min}}$. Propulsive plans are generated as linear combinations of $\Delta \delta \boldsymbol{\alpha}_i$, or $S^*(\delta v_{\text{min}},T_{\text{opt}})$, given as
\begin{align} \label{eq: optimal system}
    \begin{bmatrix}
        \Vec{\boldsymbol{1}} & \Delta \delta \boldsymbol{\alpha}^S_{\text{non-dom}}
    \end{bmatrix}^{\text{T}}
    \Vec{\boldsymbol{c}} &= 
    \begin{bmatrix}
        1 & \Delta \delta \boldsymbol{\alpha}_{\text{non-dom}}
    \end{bmatrix}^{\text{T}}
\end{align}
\noindent where $\Vec{\boldsymbol{c}} \in R^{m \times 1}$ is a column vector of $\delta v_{\text{min}}$ coefficients for $m$ maneuvers, optimality constraint $\Vec{\boldsymbol{1}} \in R^{m \times 1}$ is a column vector of ones, and $\Delta \delta \boldsymbol{\alpha}^S_{\text{non-dom}} \in R^{m \times m-1}$ concatenates values for the non-dominant ROE from $S(\delta v_{\text{min}},T_{\text{opt}})$. All plans are searched to find the combination with lowest cost. Searching is performed efficiently by restricting maneuvers to the optimal direction, tangential for IP and normal for OOP, requiring the inclusion of times that maximize efficiency in the non-dominant dimensions, guaranteeing a lowest cost maneuver plan, and considering the fewest maneuvers required for full-state controllability and minimum cost. Again, due to the coupling between 2D planes, this approach is not guaranteed to find an optimal maneuver plan. In this case, a near-optimal plan can be generated by replacing the optimality constraint with the dynamic constraint on the dominant dimension. The authors incorporated supplemental accommodations for $\delta \lambda$ dominant IP reconfigurations to ensure near-optimality with the closed-form approach and mitigated the effect of IP maneuvers on the OOP state not captured by the sequential solution process.
